Fixed Parameter Approximations for k-Center Problems in Low Highway Dimension Graphs

We consider the $k$-Center problem and some generalizations. For $k$-Center a set of $k$ center vertices needs to be found in a graph $G$ with edge lengths, such that the distance from any vertex of $G$ to its nearest center is minimized. This problem naturally occurs in transportation networks, and therefore we model the inputs as graphs with bounded highway dimension, as proposed by Abraham et al. [SODA 2010]. We show both approximation and fixed-parameter hardness results, and how to overcome them using fixed-parameter approximations, where the two paradigms are combined. In particular, we prove that for any $\varepsilon>0$ computing a $(2-\varepsilon)$-approximation is W[2]-hard for parameter $k$ and NP-hard for graphs with highway dimension $O(\log^2 n)$. The latter does not rule out fixed-parameter $(2-\varepsilon)$-approximations for the highway dimension parameter $h$, but implies that such an algorithm must have at least doubly exponential running time in $h$ if it exists, unless the ETH fails. On the positive side, we show how to get below the approximation factor of $2$ by combining the parameters $k$ and $h$: we develop a fixed-parameter $3/2$-approximation with running time $2^{O(kh\log h)}\cdot n^{O(1)}$. Additionally we prove that, unless P=NP, our techniques cannot be used to compute fixed-parameter $(2-\varepsilon)$-approximations for only the parameter $h$. We also provide similar fixed-parameter approximations for the weighted $k$-Center and $(k,\mathcal{F})$-Partition problems, which generalize $k$-Center.

==> preamble.tex <==
\usepackage{ifthen}
\usepackage{comment}
\makeatletter 
\pdfminorversion=5

\usepackage[sort,comma,square,numbers]{natbib}
\renewcommand*{\NAT@spacechar}{~} %
\renewcommand\bibsection %
{
  \section*{\refname
    \@mkboth{\MakeUppercase{\refname}}{\MakeUppercase{\refname}}}
}

%
\usepackage[margin=1in]{geometry}
%
%
%

\ifthenelse{\isundefined{\lipics}}
{
\usepackage[colorlinks=true,bookmarks=false]{hyperref}
\usepackage[small,bf]{caption}
\usepackage[pdftex]{graphicx}
\usepackage{subfigure}
\usepackage[british]{babel}
}
{}
\usepackage{xcolor}
\definecolor{darkblue}{rgb}{0,0,0.45}
\definecolor{darkred}{rgb}{0.6,0,0}
\definecolor{darkgreen}{rgb}{0.13,0.5,0}
\hypersetup{colorlinks, linkcolor=darkblue, citecolor=darkgreen, 
urlcolor=darkblue}

\ifthenelse{\isundefined{\llncs}}{
  \usepackage{amsthm}
  \usepackage{authblk}
  \renewcommand\Affilfont{\small}
}

\usepackage{amsmath,amsfonts,amssymb} 
\usepackage{mathtools}
\usepackage{mathrsfs}
\usepackage{wrapfig}
\usepackage{xspace}
\usepackage[shortlabels,inline]{enumitem}
\setlist[enumerate]{nosep}
\setlist[itemize]{nosep}


%
\usepackage[protrusion=true,expansion=true]{microtype}

\usepackage[ruled, linesnumbered, vlined]{algorithm2e}

\usepackage{aliascnt}
\ifthenelse{\isundefined{\llncs}}{
  \theoremstyle{plain} 
}{}
\newtheorem{thm}{Theorem}%
\newaliascnt{lem}{thm}
\newaliascnt{crl}{thm}
\newaliascnt{dfn}{thm}
%
\newaliascnt{prop}{thm}
\newcommand{\cqed}{\renewcommand{\qed}{\hfill$\lrcorner$}}
\newtheorem{lem}[lem]{Lemma} 
%
%
\newtheorem{crl}[crl]{Corollary} 
\ifthenelse{\isundefined{\llncs}}{
  \theoremstyle{definition} 
}{}
\newtheorem{dfn}[dfn]{Definition}
\aliascntresetthe{lem}
\aliascntresetthe{crl}
%
\aliascntresetthe{dfn}
%
%
\providecommand*{\thmautorefname}{Theorem}
\providecommand*{\lemautorefname}{Lemma}
\providecommand*{\crlautorefname}{Corollary}
\providecommand*{\dfnautorefname}{Definition}
%

%
\newcommand{\ol}[1]{{\overline{#1}}}
\newcommand{\mc}[1]{{\mathcal{#1}}}
\newcommand{\ms}[1]{\ensuremath{\mathscr{#1}}}
\newcommand{\eps}{{\varepsilon}}

\newcommand{\ignore}[1]{}
%

%
%
\usepackage{environ,xstring}
\newif\iflabel
\newif\ifdbs
\newif\ifamp
\NewEnviron{doitall}{%
  \noexpandarg
  \expandafter\IfSubStr\expandafter{\BODY}{\label}{\labeltrue}{\labelfalse}%
  \expandafter\IfSubStr\expandafter{\BODY}{\\}{\dbstrue}{\dbsfalse}%
  \expandafter\IfSubStr\expandafter{\BODY}{&}{\amptrue}{\ampfalse}%
  \iflabel\def\doitallstar{}\else\def\doitallstar{*}\fi
  \ifdbs
    \ifamp
      \def\doitallname{align}%
    \else
      \def\doitallname{multline}%
    \fi
  \else
    \def\doitallname{equation}
  \fi
  \begingroup\edef\x{\endgroup
    \noexpand\begin{\doitallname\doitallstar}%
    \noexpand\BODY
    \noexpand\end{\doitallname\doitallstar}%
  }\x
}
\def\[#1\]{\begin{doitall}#1\end{doitall}}

\makeatother 

\newcommand{\pname}[1]{\textsc{#1}}
%
%
%
%

